Are We Ready for Robust and Resilient SLAM? A Framework For Quantitative Characterization of SLAM Datasets

Reliability of SLAM systems is considered one of the critical requirements in modern autonomous systems. This directed the efforts to developing many state-of-the-art systems, creating challenging datasets, and introducing rigorous metrics to measure SLAM performance. However, the link between datasets and performance in the robustness/resilience context has rarely been explored. In order to fill this void, characterization of the operating conditions of SLAM systems is essential in order to provide an environment for quantitative measurement of robustness and resilience. In this paper, we argue that for proper evaluation of SLAM performance, the characterization of SLAM datasets serves as a critical first step. The study starts by reviewing previous efforts for quantitative characterization of SLAM datasets. Then, the problem of perturbation characterization is discussed and the linkage to SLAM robustness/resilience is established. After that, we propose a novel, generic and extendable framework for quantitative analysis and comparison of SLAM datasets. Additionally, a description of different characterization parameters is provided. Finally, we demonstrate the application of our framework by presenting the characterization results of three SLAM datasets: KITTI, EuroC-MAV, and TUM-VI highlighting the level of insights achieved by the proposed framework.

==> general_char.tex <==
\section{General Non-Sensory Metrics Characterization}
General characterizations of datasets refer to the characteristics which does not depend on the physical output of a certain sensor. Rather, they depend on the conditions of data acquisition. General characteristics are usually reported as part of the qualitative description of datasets. However, not all datasets report them. Thus, the need to automatically report these quantities becomes important in our proposed context.

\subsection{Dataset Size}
Dataset size refers to the number of sequences available and the number of sensor measurements available for each sequence. This can be extended to detect the number of scenes available as well, however, this semantic analysis is beyond the current scope of the paper. 

\subsection{Total Duration}
The total duration is calculated by accumulating the timestamps difference of the sequence. The duration is reported for each available sensor in the data acquisition set-up as an indication of the level of synchronization between different dataset sensors.

\subsection{Sensors' Sample Time}
The sample time is defined as the time step which a certain data sample represents and is reported in seconds. This can be calculated by measuring the difference between timestamps. The average sample time is an approximation usually used to represent the sensors' sampling rates, which can be calculated by:
\begin{equation}
t_{sensor} = \frac{\sum_{i=2}^{N} (t_{i} - t_{i-1}) }{N}
\end{equation}

In the proposed framework, the exact sample time is used for any differentiation/integration operations. This can lead to a better and a more accurate calculation of higher order derivatives and avoids the production of any residual errors as a result of the sample time approximations. 

\subsection{Sensors' Timestamps Mismatch}
Most of the available SLAM datasets provide their sensors' data after some level of post-processing, which usually includes removing a number of data anomalies such as timestamps mismatch. However, this is not the general case when raw data are used directly. For any multi-sensor system (such as SLAM) to operate correctly, input information must be synchronized and sampled at the exact same time to avoid any data integrity issues. In order to detect this anomaly, closest match to a certain sensor's sample time is extracted from timestamps vectors of other sensors. Then the difference in timestamps is measured and reported.

==> inertial_char.tex <==
\section{Inertial Data Characterization}
Inertial Measurement Units (IMUs) are considered a basic building block in industrial/commercial navigation systems. The reason for that, is the considerable gain in terms of accuracy that can be achieved with the integration of visual and inertial sensors. This is reflected on datasets since the introduction of the New College Dataset \cite{smith2009new} and till our current day with tens of introduced datasets in-between. Inertial characteristics of a dataset can provide information on the motion profile, the aggressiveness of motion, and the composition of motion with respect to different axes in a coordinate system. 

\subsection{Higher-Order Time Derivatives of Inertial Data}
Statistical analysis of inertial data are commonly used as an indicator of the boundaries of motion profiles. Moreover, more information can be deduced from the statistical analysis of higher order time derivatives of inertial measurements. For instance, \emph{Jerk ($j$)} and \emph{Snap $S$} \cite{schot1978jerk}, are defined to be the first and second order time-derivatives of acceleration, which are a commonly used quantities to measure the smoothness of motion and the level of sudden/abrupt changes a certain rigid body is experiencing. Similarly,  first and second order time-derivatives of angular velocity data known as the \emph{angular acceleration $\alpha$} and \emph{angular jerk $\varphi$}, are indicators of the aggressiveness and smoothness of the rotation performed by the carrier holding the system sensors.

\begin{equation}
\vec{j^b} = \frac{d \vec{f^b}}{dt} 
\qquad \qquad
\vec{S^b} = \frac{d \vec{j^b}}{dt} = \frac{d^2 \vec{f^b}}{dt^2}
\label{acc_equ}
\end{equation}

\begin{equation}
\vec{{\alpha}^b} = \frac{d \vec{{\omega}^b}}{dt}
\qquad \qquad
\vec{{\varphi}^b} = \frac{d \vec{{\alpha}^b}}{dt} = \frac{d^2 \vec{{\omega}^b}}{dt^2}
\label{angular_equ}
\end{equation}

Where: $\vec{j^b}$, $\vec{S^b}$, $\vec{{\alpha}^b}$, and $\vec{{\varphi}^b}$ are the jerk, snap, angular acceleration, and angular jerk. The quantities provided are 3-dimensional vectors representing the three sensing axes of accelerometer and gyroscope referenced to the body frame. 

Higher-order derivative of motion profiles are of great importance in modern control systems due to the reliance on them for actuating physical plants. Controlling higher-order derivatives is famous for providing more stability and robustness\cite{oliveira2020general}.

\subsection{Sensors Saturation}
Examination of the IMU measurements against its dynamic range can be used to detect the occurrence of saturation conditions, which is an indication of possible data loss due to the data clipping experienced. It is also an indication that the motion is beyond the measurable limits of the IMU, and thus an indication of the wrong choice of the sensors configuration in the dataset collection set-up.

Fig. \ref{fig:dynamic_range_fig} illustrates the importance of data saturation checking and the impact of dynamic range crossing on the reliability of the sensor data.

\subsection{Detection of Rotation-Only Motion Profiles}
Rotation-only motion profiles is the scenario where the carrier is only performing rotation around its center-of-mass with no translation in any axis, which imposes a challenge on traditional SLAM systems that rely on keyframes for motion estimation. The rotation-only motion profile forces the keyframe selection module to drop a huge number of frames, resulting in a very sparse keyframes vector which causes both the mapping and localization to fail \cite{pirchheim2013handling}. Due to this fact, SLAM datasets need to be characterized for the detection of such motion profiles. 

The detection of rotation-only motion profiles can be done either by analyzing the ground-truth localization data or the acceleration data provided as part of the dataset. The former method is straightforward and is done by extracting the translation vector of the carrier and detecting any non-zero components present. The process can be enhanced by setting a threshold to absorb the small noise margin the data acquisition system may be subject to. 

The later method depends on the principle of operation of the accelerometer itself. The accelerometer is capable of measuring any linear acceleration (in case of linear motion) and the gravity vector as well \cite{noureldin2012fundamentals}. Although the acceleration measurements are provided in the body frame, the existence of linear acceleration can be detected by measuring the total acceleration magnitude, and comparing it to the gravity value. The comparison is augmented by an uncertainty range of 10\% to avoid any acceleration noises present. This ratio is added to accommodate for both the non-idealities of the IMU, and for the compensation of the Corlios effect. The acceleration magnitude can be calculated by:

\begin{equation}
f_{magnitude} = \sqrt{f_{x,b}^2 + f_{y,b}^2 + f_{z,b}^2}
\end{equation}

Where $[f_{x,b}, f_{y,b}, f_{z,b}]^T$ is the acceleration vector in the body frame. 
The acceleration magnitude $f_{magnitude}$ is then tested to detect linear translation as follows:

\begin{equation}
T_{status} = 
\begin{cases}
    1, & \text{if } f_{magnitude}\leq 9.81\pm10\%\\
    0, & \text{otherwise}
\end{cases}
\end{equation}


==> plots/ds_plots_col.tex <==
% Entropy Plot
\begin{figure}[H]
     \centering
     \begin{subfigure}[]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/H_general.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/H_inertial.png}
     \end{subfigure}      
	 \\ 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/H_visual.png}
     \end{subfigure}
     \hfill
        \caption{Entropy Analysis Results}
        \label{fig:H_fig_col}
\end{figure}

% SDI Plot
\begin{figure}[H]
     \centering
     \begin{subfigure}[]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/SDI_general.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[]{0.62\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/SDI_inertial.png}
     \end{subfigure}      
	 \\ 
     \begin{subfigure}[]{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/SDI_visual.png}
     \end{subfigure}
     \hfill
        \caption{Simpson's Diversity Analysis Results}
        \label{fig:SDI_fig_col}
\end{figure}

==> plots/ds_plots_detailed_res_inertial.tex <==
%\begin{figure}[H]
%     \centering
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_AX.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_AY.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_AZ.png}
%     \end{subfigure}
%	 \\ 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_AX.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_AY.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_AZ.png}
%     \end{subfigure}
%        \caption{Accelerometer Characterization Results}
%        \label{fig:inertial_1_fig}
%\end{figure}

\begin{figure}[H]
     \centering
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_GX.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_GY.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_GZ.png}
     \end{subfigure}
	 \\ 
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_GX.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_GY.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_GZ.png}
     \end{subfigure}
        \caption{Gyroscope Characterization Results}
        \label{fig:inertial_2_fig}
\end{figure}

\begin{figure}[H]
     \centering
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_ACC_MAG.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_ACC_MAG.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/rot_only_percent.png}
     \end{subfigure}
        \caption{Rotation-Only Motion Characterization Results}
        \label{fig:inertial_3_fig}
\end{figure}

==> plots/ds_plots_detailed_res_visual.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Contrast
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
     \centering
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_CONTRAST_CR.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_CONTRAST_WEBER.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_CONTRAST_MICHELSON.png}
     \end{subfigure}
     \hfill
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_CONTRAST_RMS.png}
     \end{subfigure}
     \\
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_CONTRAST_CR.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_CONTRAST_WEBER.png}
     \end{subfigure}    
     \hfill     
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_CONTRAST_MICHELSON.png}
     \end{subfigure}
     \hfill  
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_CONTRAST_RMS.png}
     \end{subfigure}
        \caption{Contrast Characterization Results}
        \label{fig:contrast_fig}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Brightness
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
     \centering
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_BRIGHTNESS.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_BRIGHTNESS.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/brightness_diff.png}
     \end{subfigure}
        \caption{Brightness Characterization Results}
        \label{fig:brightness_fig}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Detectable Features
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[H]
%     \centering
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_SIFT_COUNT.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_SIFT_DIST_ABS.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_SIFT_DIST_AVG.png}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_SIFT_COUNT.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_SIFT_DIST_ABS.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_SIFT_DIST_AVG.png}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_ORB_COUNT.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_ORB_DIST_ABS.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_ORB_DIST_AVG.png}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_ORB_COUNT.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_ORB_DIST_ABS.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_ORB_DIST_AVG.png}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_FAST_COUNT.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_FAST_DIST_ABS.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_FAST_DIST_AVG.png}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_FAST_COUNT.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_FAST_DIST_ABS.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.31\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_FAST_DIST_AVG.png}
%     \end{subfigure}
%        \caption{Detectable Feature Characterization Results}
%        \label{fig:detectable_VF_fig}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Disparity
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[H]
%     \centering
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_DISPARITY_AVG_BM.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_DISPARITY_STD_DIV_BM.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_DISPARITY_AVG_SGBM.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_DISPARITY_STD_DIV_SGBM.png}
%     \end{subfigure}
%	\\  
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_DISPARITY_AVG_BM.png}
%     \end{subfigure}
%     \hfill 
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_DISPARITY_STD_DIV_BM.png}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_DISPARITY_AVG_SGBM.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.24\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_DISPARITY_STD_DIV_SGBM.png}
%     \end{subfigure}
%        \caption{Disparity Characterization Results}
%        \label{fig:disparity_fig}
%\end{figure}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Revisit Frequency
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[H]
%     \centering
%     \begin{subfigure}[H]{0.49\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_REVISIT_SCORE.png}
%     \end{subfigure}
%     \hfill     
%     \begin{subfigure}[H]{0.49\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_REVISIT_SCORE.png}
%     \end{subfigure}
%        \caption{Image Similarity Characterization Results}
%        \label{fig:revisit_fig}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Exposure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
     \centering
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_EXPOSURE_MEAN.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_EXPOSURE_MEAN.png}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[H]{0.31\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/exposure_percent_barchart.png}
     \end{subfigure}
        \caption{Exposure Characterization Results}
        \label{fig:exposure_fig}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Blurring
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]
     \centering
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_BLUR_SCORE.png}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_BLUR_SCORE.png}
     \end{subfigure}
     \hfill 
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/raincloud_figs/raincloud_BLUR_PERCENT.png}
     \end{subfigure}
	\hfill  
     \begin{subfigure}[H]{0.24\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/KDEplot_figs/KDE_BLUR_PERCENT.png}
     \end{subfigure}
     \caption{Image Blurring Characterization Results}
        \label{fig:blur_fig}
\end{figure}









==> robustness_resilience.tex <==
% =====================================================================================================
\section{Accuracy vs. Robustness vs. Resilience}
Accuracy, being defined as the deviation of the system output from a reference output, was quantitatively defined, which was evident in the availability of accuracy performance metrics such as the \emph{Absolute Trajectory Error (ATE)} and \emph{Relative Trajectory Error (RTE)} \cite{zhang2018tutorial}, and the study of their statistical relation to each other \cite{zhang2019rethinking}. Robustness and Resilience, on the other hand, were not properly-defined or measured in the SLAM context, and the two terms were used loosely as an indication of accuracy despite their importance in the modern SLAM era \cite{cadena2016past}. Consequently, the SLAM community lacks a robustness/resilience-aware comparisons of SLAM systems. One way to have a rigorous definition of the two terms is to conduct comparative analogies to other disciplines where the two terms are well-defined, measured, and utilized. 

The term \textbf{Robustness} is of great importance in the SLAM context due to the criticality of the information a SLAM system can provide. Robustness is defined as the ability of the system to maintain a certain level of accuracy under a defined level of perturbations. The term is widely used in a number of areas other than SLAM. For instance, in \emph{Biological Systems}, robustness is defined as the ability to maintain a certain characteristic or performance under uncertainty or perturbations \cite{stelling2004robustness}\cite{felix2008robustness}. The term is also very popular in \emph{Systems Engineering}, where it is defined to be The ability of the system to maintain acceptable performance across requirement spectrum, with adaptability to new scenarios, and while having internal error tolerance mechanisms \cite{sussman2007building}. In \emph{Electro-Mechanical Systems}, the same term is defined to be The ability of a system (e.g. control loop) to maintain performance within required specs and stability, under plant perturbations \cite{steinbuch1991robustness}\cite{stoten1990robustness}.

Similar to robustness, the term \textbf{Resilience} is also a widely used term in the SLAM literature, and is used interchangeably with robustness as one can observe in\cite{thyagharajan2020towards} \cite{balcilar2017r}. The problem of resilience in robotics was discussed in \cite{prorok2021beyond}, and the difference between robustness and resilience was illustrated thoroughly. Resilience is the ability of the system to adapt, tolerate, or recover from out-of-range perturbations. This definition highlights the importance of perturbations characterization and how this can be used to measure the resilience of SLAM systems. This definition aligns firmly with the definition of resilience in other disciplines such as .

% =====================================================================================================
\subsection*{Measuring Robustness and Resilience of SLAM Systems}
Robustness and Resilience in SLAM are tightly coupled with the characterization and quantification of the perturbations the system is subject to \cite{prorok2021beyond}. The perturbations to SLAM systems come in two main categories: perturbation in the form of pre-recorded datasets and benchmarks, and real-time perturbation after deploying a real robot in a physical environment. The former method is widely used in the context of development, validation, and performance comparison despite the lack of quantitative characterization to the data used. 

Quantitative measurement robustness and resilience is not a trivial task due to the wide spectrum of aspects a certain system shall be immune to. Several trials were proposed to measure robustness based on the associated datasets \cite{bujanca2021robust}. However, with no quantification of the perturbations, a quantitative measure of robustness and resilience cannot be realized. From the trajectory accuracy perspective, \emph{Absolute Trajectory Error (ATE)} and \emph{Relative Trajectory Error (RTE)} \cite{zhang2018tutorial}, are claimed to be non-sufficient for the measurement of robustness and resilience, which is true given the lack of a measurement for the associated operating ranges. With the existence of such metrics, a link can be established between accuracy and the associated operating conditions. From the robustness perspective, one can provide performance guarantees within a certain perturbation levels (operating conditions). Consequently, one can measure resilience by exposing the SLAM system to conditions outside of the defined operating conditions until divergence is witnessed. The measurement of the re-convergence of the system and the accuracy after re-convergence is a direct indication of resilience of the system.

==> sat_fig.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/dynamic_range/noSat_fig.png}
         \caption{}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/dynamic_range/sat_fig.png}
         \caption{}
     \end{subfigure}
        \caption{An example of inertial sensor saturation and data loss anomaly. (a) Represents a physical signal within the sensor dynamic range. (b) Represents a physical signal beyond the sensor's dynamic range and illustrating the data clipping/loss witnessed}
        \label{fig:dynamic_range_fig}
\end{figure}

==> tables/H_SDI_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[!htpb]
\caption{Entropy and Diversity Analysis Results}
\label{tab:H_SDI_table}
\begin{subtable}[]{\columnwidth}
\label{tab:ds_H_SDI_general}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcc|cc|cc@{}}
%%%%%%%%%%%%%%
\cmidrule(l){2-7} &
  \multicolumn{2}{c|}{KITTI} &
  \multicolumn{2}{c|}{EuroC} &
  \multicolumn{2}{c}{TUM-VI}  \\ \toprule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{\textbf{Analysis Metric}} &
  $H$ & $SDI$ &
  $H$ & $SDI$ &
  $H$ & $SDI$ \\ \bottomrule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{Samples (RGB - L) [$Samples$]} & 2.941 & 0.987 & 2.398 & 1.0 & 3.283 & 0.997 \\
\multicolumn{1}{l||}{Samples (RGB - R) [$Samples$]} & 2.941 & 0.987 & 2.398 & 1.0 & 3.283 & 0.997 \\
\multicolumn{1}{l||}{Samples (IMU) [$Samples$]} & 0 & 0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Seq. Duration (RGB - L) [$sec$]} & 3.091 & 1.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Seq. Duration (RGB - R) [$sec$]} & 3.091 & 1.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Seq. Duration (IMU) [$sec$]} & 0 & 0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Sample Time (RGB - L) [$sec$]} & 3.96 & 0.948 & 0.988 & 0.598 & 2.876 & 0.845 \\
\multicolumn{1}{l||}{Sample Time (RGB - R) [$sec$]} & 3.96 & 0.948 & 1.06 & 0.609 & 2.876 & 0.845 \\
\multicolumn{1}{l||}{Sample Time (IMU) [$sec$]} & 0 & 0 & 0.895 & 0.55 & 2.516 & 0.897 \\
\multicolumn{1}{l||}{V-I TS Mismatch [$sec$]} & 0 & 0 & 0.001 & 0.0 & 9.916 & 1.0 \\
\bottomrule
\end{tabular}
}
\caption{General Characterization Metrics}
\end{subtable}

\begin{subtable}[]{\columnwidth}
\label{tab:ds_H_SDI_inertial}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcc|cc|cc@{}}
%%%%%%%%%%%%%%
\cmidrule(l){2-7} &
  \multicolumn{2}{c|}{KITTI} &
  \multicolumn{2}{c|}{EuroC} &
  \multicolumn{2}{c}{TUM-VI}  \\ \toprule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{\textbf{Analysis Metric}} &
  $H$ & $SDI$ &
  $H$ & $SDI$ &
  $H$ & $SDI$ \\ \bottomrule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{Ax [$m/sec^2$]} & 0 & 0 & 6.493 & 0.998 & 8.111 & 1.0 \\
\multicolumn{1}{l||}{Ay [$m/sec^2$]} & 0 & 0 & 5.691 & 0.996 & 12.531 & 1.0 \\
\multicolumn{1}{l||}{Az [$m/sec^2$]} & 0 & 0 & 6.111 & 0.997 & 12.575 & 1.0 \\
\multicolumn{1}{l||}{Gx [$deg/sec$]} & 0 & 0 & 7.12 & 0.998 & 14.109 & 1.0 \\
\multicolumn{1}{l||}{Gy [$deg/sec$]} & 0 & 0 & 7.042 & 0.999 & 14.196 & 1.0 \\
\multicolumn{1}{l||}{Gz [$deg/sec$]} & 0 & 0 & 6.959 & 0.999 & 14.078 & 1.0 \\
\multicolumn{1}{l||}{$d Ax/ dt$ [$m/sec^3$]} & 0 & 0 & 7.711 & 0.999 & 7.952 & 0.999 \\
\multicolumn{1}{l||}{$d Ay/ dt$ [$m/sec^3$]} & 0 & 0 & 6.748 & 0.998 & 11.507 & 1.0 \\
\multicolumn{1}{l||}{$d Az/ dt$ [$m/sec^3$]} & 0 & 0 & 7.304 & 0.999 & 14.032 & 1.0 \\
\multicolumn{1}{l||}{$d Gx/ dt$ [$deg/sec^2$]} & 0 & 0 & 5.826 & 0.996 & 13.501 & 1.0 \\
\multicolumn{1}{l||}{$d Gy/ dt$ [$deg/sec^2$]} & 0 & 0 & 7.038 & 0.999 & 13.633 & 1.0 \\
\multicolumn{1}{l||}{$d Gz/ dt$ [$deg/sec^2$]} & 0 & 0 & 6.425 & 0.998 & 14.058 & 1.0 \\
\multicolumn{1}{l||}{$d Ax^2/ dt^2$ [$m/sec^4$]} & 0 & 0 & 10.496 & 1.0 & 11.58 & 1.0 \\
\multicolumn{1}{l||}{$d Ay^2/ dt^2$ [$m/sec^4$]} & 0 & 0 & 9.861 & 1.0 & 12.096 & 1.0 \\
\multicolumn{1}{l||}{$d Az^2/ dt^2$ [$m/sec^4$]} & 0 & 0 & 10.197 & 1.0 & 13.998 & 1.0 \\
\multicolumn{1}{l||}{$d Gx^2/ dt^2$ [$deg/sec^4$]} & 0 & 0 & 8.879 & 1.0 & 12.766 & 1.0 \\
\multicolumn{1}{l||}{$d Gy^2/ dt^2$ [$deg/sec^4$]} & 0 & 0 & 9.957 & 1.0 & 12.743 & 1.0 \\
\multicolumn{1}{l||}{$d Gz^2/ dt^2$ [$deg/sec^4$]} & 0 & 0 & 9.405 & 1.0 & 13.753 & 1.0 \\
\multicolumn{1}{l||}{Ax DR Coverage [$\%$]} & 0.0 & 0.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Ay DR Coverage [$\%$]} & 0.0 & 0.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Az DR Coverage [$\%$]} & 0.0 & 0.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Gx DR Coverage [$\%$]} & 0.0 & 0.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Gy DR Coverage [$\%$]} & 0.0 & 0.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Gz DR Coverage [$\%$]} & 0.0 & 0.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Acc. Magnitude [$m/sec^2$]} & 0 & 0 & 10.835 & 1.0 & 12.473 & 1.0 \\
\multicolumn{1}{l||}{Rotation Only Motion [$\%$]} & 0 & 0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\bottomrule
\end{tabular}
}
\caption{Inertial Characterization Metrics}
\end{subtable}


\begin{subtable}[]{\columnwidth}
\label{tab:ds_H_SDI_visual}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lcc|cc|cc@{}}
%%%%%%%%%%%%%%
\cmidrule(l){2-7} &
  \multicolumn{2}{c|}{KITTI} &
  \multicolumn{2}{c|}{EuroC} &
  \multicolumn{2}{c}{TUM-VI}  \\ \toprule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{\textbf{Analysis Metric}} &
  $H$ & $SDI$ &
  $H$ & $SDI$ &
  $H$ & $SDI$ \\ \bottomrule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{Brightness [$DL$]} & 10.508 & 1.0 & 10.101 & 1.0 & 12.298 & 1.0 \\
\multicolumn{1}{l||}{d Br/dt [$DL$]} & 10.666 & 1.0 & 10.194 & 1.0 & 12.45 & 1.0 \\
\multicolumn{1}{l||}{d Br/d $>$ 1$\sigma$ [$\%$]} & 3.091 & 1.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{d Br/d $>$ 2$\sigma$ [$\%$]} & 3.091 & 1.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{d Br/d $>$ 3$\sigma$ [$\%$]} & 3.091 & 1.0 & 2.398 & 1.0 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Black Exposure [$\%$]} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\multicolumn{1}{l||}{White Exposure [$\%$]} & 0.0 & 0.0 & 0.0 & 0.0 & 0.154 & 0.071 \\
\multicolumn{1}{l||}{Over Exposure [$\%$]} & 0.0 & 0.0 & 0.0 & 0.0 & 0.458 & 0.206 \\
\multicolumn{1}{l||}{Proper Exposure [$\%$]} & 0.0 & 0.0 & 1.16 & 0.618 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Under Exposure [$\%$]} & 0.0 & 0.0 & 1.16 & 0.618 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Exposure Img. Mean [$DL$]} & 10.524 & 1.0 & 10.07 & 1.0 & 12.281 & 1.0 \\
\multicolumn{1}{l||}{Exposure Img. Skewness [$DL$]} & 10.508 & 1.0 & 10.172 & 1.0 & 12.22 & 1.0 \\
\multicolumn{1}{l||}{Exposure Zone [$DL$]} & 0.17 & 0.076 & 0.946 & 0.564 & 0.971 & 0.581 \\
\multicolumn{1}{l||}{Contrast Ratio [$DL$]} & 9.351 & 1.0 & 9.8 & 1.0 & 10.021 & 1.0 \\
\multicolumn{1}{l||}{Weber Contrast Score [$DL$]} & 10.501 & 1.0 & 10.182 & 1.0 & 12.079 & 1.0 \\
\multicolumn{1}{l||}{Michelson Contrast Score [$DL$]} & 1.949 & 0.818 & 1.33 & 0.518 & 1.064 & 0.549 \\
\multicolumn{1}{l||}{RMS Contrast Score [$DL$]} & 10.601 & 1.0 & 10.157 & 1.0 & 12.234 & 1.0 \\
\multicolumn{1}{l||}{Blurring Percentage  [$\%$]} & 4.28 & 0.984 & 4.222 & 0.979 & 4.582 & 0.989 \\
\multicolumn{1}{l||}{Blurring Score [$DL$]} & 10.625 & 1.0 & 10.178 & 1.0 & 12.272 & 1.0 \\
\multicolumn{1}{l||}{Local Blurring ($>$0\%) [$\%$]} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\multicolumn{1}{l||}{Blurred Images ($>$ 50\%) [$\%$]} & 0.902 & 0.411 & 2.272 & 0.982 & 3.332 & 1.0 \\
\multicolumn{1}{l||}{Global Blurring ($>$90\%) [$\%$]} & 0.0 & 0.0 & 0.305 & 0.182 & 3.134 & 0.984 \\
\multicolumn{1}{l||}{No. SIFT Features [$Features$]} & 8.218 & 1.0 & 7.927 & 1.0 & 7.552 & 0.999 \\
\multicolumn{1}{l||}{Abs. Spatial Dist. - SIFT [$\%$]} & 8.16 & 1.0 & 7.239 & 0.999 & 6.823 & 0.999 \\
\multicolumn{1}{l||}{Avg. Spatial Dist. - SIFT [$\%$]} & 8.307 & 1.0 & 7.433 & 0.999 & 6.792 & 0.999 \\
\multicolumn{1}{l||}{No. ORB Features [$Features$]} & 9.101 & 1.0 & 9.015 & 1.0 & 9.042 & 1.0 \\
\multicolumn{1}{l||}{Abs. Spatial Dist. - ORB [$\%$]} & 8.004 & 1.0 & 7.174 & 0.999 & 6.971 & 0.999 \\
\multicolumn{1}{l||}{Avg. Spatial Dist.- ORB [$\%$]} & 8.127 & 1.0 & 7.169 & 0.999 & 6.692 & 0.999 \\
\multicolumn{1}{l||}{No. FAST Features [$Features$]} & 9.217 & 1.0 & 8.804 & 1.0 & 8.753 & 1.0 \\
\multicolumn{1}{l||}{Abs. Spatial Dist. - FAST [$\%$]} & 8.102 & 1.0 & 7.504 & 0.999 & 7.446 & 0.999 \\
\multicolumn{1}{l||}{Avg. Spatial Dist. - FAST [$\%$]} & 8.041 & 1.0 & 7.34 & 0.999 & 7.083 & 0.999 \\
\multicolumn{1}{l||}{Disparity Mean (BM) [$DL$]} & 10.566 & 1.0 & 10.138 & 1.0 & 12.097 & 1.0 \\
\multicolumn{1}{l||}{Disparity Std. Dev. (BM) [$DL$]} & 10.598 & 1.0 & 10.148 & 1.0 & 12.062 & 1.0 \\
\multicolumn{1}{l||}{Disparity Mean (SGBM) [$DL$]} & 10.589 & 1.0 & 10.156 & 1.0 & 12.134 & 1.0 \\
\multicolumn{1}{l||}{Disparity Std. Dev. (SGBM) [$DL$]} & 10.609 & 1.0 & 10.172 & 1.0 & 12.151 & 1.0 \\
\multicolumn{1}{l||}{Dist to Closest Match [$Samples$]} & 0.709 & 0.167 & 0.895 & 0.318 & 0.612 & 0.227 \\
\multicolumn{1}{l||}{Image Similarity Score [$DL$]} & 10.203 & 1.0 & 9.733 & 1.0 & 11.527 & 1.0 \\
\bottomrule
\end{tabular}
}
\caption{Visual Characterization Metrics}
\end{subtable}
\end{table}

==> tables/metrics_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\caption{Summary of Characterization Metrics Included in DS-EVAL}
\label{tab:metrics_table}
%\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|l|l|l|l|l@{}}
\toprule
\textbf{ID} & \textbf{Metric} & \textbf{Unit} & \textbf{Definition} & \textbf{Parameters} & \textbf{Description} \\ \midrule
G01 & \# Sequences        & DN &  &  &  \\
    & \# Visual Samples   & DN &  &  &  \\
    & \# Inertial Samples & DN &  &  &  \\ \midrule
I01 &                     &    &  &  &  \\
    &                     &    &  &  &  \\ \midrule
V01 &                     &    &  &  &  \\
    &                     &    &  &  &  \\ \bottomrule
\end{tabular}
%}
\end{table*}

==> tables/pre_work_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\newcolumntype{L}{>{\arraybackslash}m{8cm}}

\begin{table*}[]
\caption{Summary of Previous Trials of Quantitative Dataset Characterization}
\label{tab:pre-work}
\renewcommand{\arraystretch}{1.5}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}clcL@{}}
\toprule
\multicolumn{1}{c}{\textbf{Study}} &
  \multicolumn{1}{c}{\textbf{Characterization Metric}} &
  \multicolumn{1}{l}{\textbf{DAQ Status}} &
  \multicolumn{1}{c}{\textbf{Objective}} \\ \midrule
 
\cite{andreopoulos2011sensor} 
 &
  Performance under camera/scene parameter changes &
  Pre-DAQ &
  Measure computer vision algorithms performance while changing shutter speed/gain simultanously with illumination changes \\
  
  \cite{saeedi2019characterizing}
 &
  Wasserstein distance &
  Post-DAQ &
  Measure the difficulty of a dataset without depending on running a SLAM system \\
  
  \cite{Delmerico19icra}
 &
  Magnitude of Optical Flow &
  Post-DAQ &
  Measure the aggressiveness of the motion profile the camera is subject to due to the motion of the carrier \\
  
  \cite{tsotsos2019does}
 &
  Performance balance under changing camera parameters &
  Pre-DAQ &
  Prove the existence of performance imbalance while changing camera parameters (shutter speed, ISO, and gain) \\
  
  \cite{tartanair2020iros}
 &
  PCA of Motion Axes &
  Post-DAQ &
  Measure the distribution of motion profile among different axes as an indication of the complexity of motion \\ \bottomrule
\end{tabular}
}
\end{table*}

==> tables/stats_table.tex <==
\begin{table}[!htpb]
\caption{Statistical Analysis Results}
\label{tab:stats_table}
\begin{subtable}[]{\columnwidth}
\label{tab:ds_nonCounting_general}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}cc|c|c||c@{}}
%%%%%%%%%%%%%%
\cmidrule(l){2-5} & 
KITTI & 
EuroC & 
TUM-VI & 
\textbf{Aggregated} \\ \toprule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{\textbf{Analysis Metric}} 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ \\ \bottomrule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{Samples (RGB - L) [$Samples$]} & 1979.636 $\pm$ (1460.376)&2496.636 $\pm$ (548.91)&10356.893 $\pm$ (7562.473)&5918.164 $\pm$ (6600.077)\\
\multicolumn{1}{l||}{Samples (RGB - R) [$Samples$]} & 1979.636 $\pm$ (1460.376)&2459.0 $\pm$ (574.672)&10356.929 $\pm$ (7562.483)&5911.393 $\pm$ (6604.051)\\
\multicolumn{1}{l||}{Samples (IMU) [$Samples$]} & - $\pm$ (-)&24968.091 $\pm$ (5489.999)&103268.25 $\pm$ (75419.389)&81183.59 $\pm$ (72963.254)\\
\multicolumn{1}{l||}{Seq. Duration (RGB - L) [$sec$]} & 205.331 $\pm$ (151.546)&124.782 $\pm$ (27.445)&517.811 $\pm$ (378.136)&334.239 $\pm$ (319.953)\\
\multicolumn{1}{l||}{Seq. Duration (RGB - R) [$sec$]} & 205.331 $\pm$ (151.546)&124.782 $\pm$ (27.448)&517.813 $\pm$ (378.137)&334.24 $\pm$ (319.954)\\
\multicolumn{1}{l||}{Seq. Duration (IMU) [$sec$]} & - $\pm$ (-)&124.835 $\pm$ (27.45)&517.862 $\pm$ (378.132)&407.008 $\pm$ (365.917)\\
\multicolumn{1}{l||}{Sample Time (RGB - L) [$sec$]} & 0.104 $\pm$ (0.0)&0.05 $\pm$ (0.0)&0.05 $\pm$ (0.0)&0.056 $\pm$ (0.018)\\
\multicolumn{1}{l||}{Sample Time (RGB - R) [$sec$]} & 0.104 $\pm$ (0.0)&0.051 $\pm$ (0.006)&0.05 $\pm$ (0.0)&0.057 $\pm$ (0.018)\\
\multicolumn{1}{l||}{Sample Time (IMU) [$sec$]} & - $\pm$ (-)&0.005 $\pm$ (0.0)&0.005 $\pm$ (0.0)&0.005 $\pm$ (0.0)\\
\multicolumn{1}{l||}{V-I TS Mismatch [$sec$]} & - $\pm$ (-)&-0.0 $\pm$ (0.0)&0.0 $\pm$ (0.001)&0.0 $\pm$ (0.001)\\ 
\bottomrule
\end{tabular}
}
\caption{General Characterization Metrics}
\end{subtable}


\begin{subtable}[]{\columnwidth}
\label{tab:ds_nonCounting_inertial}
\centering

\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}cc|c|c||c@{}}
%%%%%%%%%%%%%%
\cmidrule(l){2-5} & 
KITTI & 
EuroC & 
TUM-VI & 
\textbf{Aggregated} \\ \toprule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{\textbf{Analysis Metric}} 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ \\ \bottomrule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{Ax [$m/sec^2$]} & - $\pm$ (-)&9.203 $\pm$ (1.378)&-0.039 $\pm$ (1.405)&0.763 $\pm$ (2.955)\\
\multicolumn{1}{l||}{Ay [$m/sec^2$]} & - $\pm$ (-)&-0.007 $\pm$ (0.605)&-0.802 $\pm$ (1.496)&-0.733 $\pm$ (1.458)\\
\multicolumn{1}{l||}{Az [$m/sec^2$]} & - $\pm$ (-)&-3.328 $\pm$ (0.96)&9.592 $\pm$ (2.26)&8.471 $\pm$ (4.239)\\
\multicolumn{1}{l||}{Gx [$deg/sec$]} & - $\pm$ (-)&0.769 $\pm$ (17.244)&-1.521 $\pm$ (21.843)&-1.322 $\pm$ (21.493)\\
\multicolumn{1}{l||}{Gy [$deg/sec$]} & - $\pm$ (-)&1.53 $\pm$ (16.888)&0.104 $\pm$ (27.857)&0.228 $\pm$ (27.085)\\
\multicolumn{1}{l||}{Gz [$deg/sec$]} & - $\pm$ (-)&4.18 $\pm$ (11.848)&0.319 $\pm$ (31.696)&0.654 $\pm$ (30.51)\\
\multicolumn{1}{l||}{$d Ax/ dt$ [$m/sec^3$]} & - $\pm$ (-)&0.0 $\pm$ (388.233)&0.001 $\pm$ (14.186)&0.001 $\pm$ (115.143)\\
\multicolumn{1}{l||}{$d Ay/ dt$ [$m/sec^3$]} & - $\pm$ (-)&0.001 $\pm$ (144.628)&-0.0 $\pm$ (15.458)&-0.0 $\pm$ (45.085)\\
\multicolumn{1}{l||}{$d Az/ dt$ [$m/sec^3$]} & - $\pm$ (-)&0.001 $\pm$ (259.104)&-0.0 $\pm$ (29.16)&-0.0 $\pm$ (81.24)\\
\multicolumn{1}{l||}{$d Gx/ dt$ [$deg/sec^2$]} & - $\pm$ (-)&-0.0 $\pm$ (283.19)&0.011 $\pm$ (248.509)&0.01 $\pm$ (251.706)\\
\multicolumn{1}{l||}{$d Gy/ dt$ [$deg/sec^2$]} & - $\pm$ (-)&-0.011 $\pm$ (960.281)&0.002 $\pm$ (246.411)&0.001 $\pm$ (368.022)\\
\multicolumn{1}{l||}{$d Gz/ dt$ [$deg/sec^2$]} & - $\pm$ (-)&0.002 $\pm$ (513.015)&0.013 $\pm$ (187.275)&0.012 $\pm$ (234.22)\\
\multicolumn{1}{l||}{$d Ax^2/ dt^2$ [$m/sec^4$]} & - $\pm$ (-)&0.247 $\pm$ (147174.077)&0.056 $\pm$ (1984.225)&0.072 $\pm$ (43386.669)\\
\multicolumn{1}{l||}{$d Ay^2/ dt^2$ [$m/sec^4$]} & - $\pm$ (-)&-0.106 $\pm$ (49896.859)&0.029 $\pm$ (1612.564)&0.017 $\pm$ (14776.034)\\
\multicolumn{1}{l||}{$d Az^2/ dt^2$ [$m/sec^4$]} & - $\pm$ (-)&-0.007 $\pm$ (98187.569)&-0.006 $\pm$ (2243.73)&-0.006 $\pm$ (28997.257)\\
\multicolumn{1}{l||}{$d Gx^2/ dt^2$ [$deg/sec^4$]} & - $\pm$ (-)&0.447 $\pm$ (71059.169)&0.193 $\pm$ (10060.189)&0.215 $\pm$ (23030.725)\\
\multicolumn{1}{l||}{$d Gy^2/ dt^2$ [$deg/sec^4$]} & - $\pm$ (-)&-0.934 $\pm$ (358726.81)&0.025 $\pm$ (11847.176)&-0.058 $\pm$ (106255.903)\\
\multicolumn{1}{l||}{$d Gz^2/ dt^2$ [$deg/sec^4$]} & - $\pm$ (-)&0.748 $\pm$ (178750.777)&0.046 $\pm$ (7676.819)&0.107 $\pm$ (53153.792)\\
\multicolumn{1}{l||}{Ax DR Coverage [$\%$]} & 0.0 $\pm$ (0.0)&10.77 $\pm$ (6.805)&5.829 $\pm$ (1.155)&4.618 $\pm$ (4.875)\\
\multicolumn{1}{l||}{Ay DR Coverage [$\%$]} & 0.0 $\pm$ (0.0)&3.597 $\pm$ (1.46)&4.202 $\pm$ (1.058)&2.577 $\pm$ (2.172)\\
\multicolumn{1}{l||}{Az DR Coverage [$\%$]} & 0.0 $\pm$ (0.0)&4.936 $\pm$ (2.7)&4.721 $\pm$ (1.503)&3.057 $\pm$ (2.756)\\
\multicolumn{1}{l||}{Gx DR Coverage [$\%$]} & 0.0 $\pm$ (0.0)&5.883 $\pm$ (1.136)&7.778 $\pm$ (2.538)&4.631 $\pm$ (3.986)\\
\multicolumn{1}{l||}{Gy DR Coverage [$\%$]} & 0.0 $\pm$ (0.0)&10.529 $\pm$ (3.473)&10.953 $\pm$ (3.271)&6.926 $\pm$ (5.862)\\
\multicolumn{1}{l||}{Gz DR Coverage [$\%$]} & 0.0 $\pm$ (0.0)&7.337 $\pm$ (2.01)&9.497 $\pm$ (1.453)&5.682 $\pm$ (4.556)\\
\multicolumn{1}{l||}{Acc. Magnitude [$m/sec^2$]} & - $\pm$ (-)&13.465 $\pm$ (1.965)&9.813 $\pm$ (2.182)&10.13 $\pm$ (2.395)\\
\multicolumn{1}{l||}{Rotation Only Motion [$\%$]} & - $\pm$ (-)&7.613 $\pm$ (2.924)&70.369 $\pm$ (8.704)&52.668 $\pm$ (29.573)\\ 
\bottomrule
\end{tabular}
}
\caption{Inertial Characterization Metrics}
\end{subtable}


\begin{subtable}[]{\columnwidth}
\label{tab:ds_nonCounting_visual}
\centering

\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}cc|c|c||c@{}}
%%%%%%%%%%%%%%
\cmidrule(l){2-5} & 
KITTI & 
EuroC & 
TUM-VI & 
\textbf{Aggregated} \\ \toprule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{\textbf{Analysis Metric}} 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ 
& $\mu \pm (\sigma)$ \\ \bottomrule
%%%%%%%%%%%%%%
\multicolumn{1}{l||}{Brightness [$DL$]} & 92.099 $\pm$ (6.606)&102.515 $\pm$ (33.344)&68.948 $\pm$ (28.159)&74.262 $\pm$ (29.11)\\
\multicolumn{1}{l||}{d Br/dt [$DL$]} & -0.001 $\pm$ (27.78)&0.296 $\pm$ (80.858)&-0.116 $\pm$ (57.452)&-0.071 $\pm$ (56.905)\\
\multicolumn{1}{l||}{d Br/d $>$ 1$\sigma$ [$\%$]} & 22.631 $\pm$ (3.332)&10.316 $\pm$ (2.088)&6.546 $\pm$ (1.074)&13.027 $\pm$ (7.74)\\
\multicolumn{1}{l||}{d Br/d $>$ 2$\sigma$ [$\%$]} & 5.597 $\pm$ (0.554)&4.332 $\pm$ (1.221)&3.296 $\pm$ (0.987)&4.313 $\pm$ (1.371)\\
\multicolumn{1}{l||}{d Br/d $>$ 3$\sigma$ [$\%$]} & 1.681 $\pm$ (0.415)&2.353 $\pm$ (0.681)&2.032 $\pm$ (0.678)&1.963 $\pm$ (0.635)\\
\multicolumn{1}{l||}{Black Exposure [$\%$]} & 0.0 $\pm$ (0.0)&0.0 $\pm$ (0.0)&0.0 $\pm$ (0.0)&0.0 $\pm$ (0.0)\\
\multicolumn{1}{l||}{White Exposure [$\%$]} & 0.0 $\pm$ (0.0)&0.0 $\pm$ (0.0)&0.0 $\pm$ (0.002)&0.0 $\pm$ (0.001)\\
\multicolumn{1}{l||}{Over Exposure [$\%$]} & 0.0 $\pm$ (0.0)&0.0 $\pm$ (0.0)&0.005 $\pm$ (0.018)&0.002 $\pm$ (0.012)\\
\multicolumn{1}{l||}{Proper Exposure [$\%$]} & 100.0 $\pm$ (0.0)&97.837 $\pm$ (4.698)&53.234 $\pm$ (23.548)&78.143 $\pm$ (28.09)\\
\multicolumn{1}{l||}{Under Exposure [$\%$]} & 0.0 $\pm$ (0.0)&2.163 $\pm$ (4.698)&46.761 $\pm$ (23.552)&21.854 $\pm$ (28.089)\\
\multicolumn{1}{l||}{Exposure Img. Mean [$DL$]} & 91.731 $\pm$ (6.822)&109.547 $\pm$ (27.025)&71.653 $\pm$ (26.004)&76.921 $\pm$ (27.072)\\
\multicolumn{1}{l||}{Exposure Img. Skewness [$DL$]} & 0.987 $\pm$ (0.302)&0.766 $\pm$ (0.685)&2.07 $\pm$ (1.457)&1.841 $\pm$ (1.404)\\
\multicolumn{1}{l||}{Exposure Zone [$DL$]} & 2.04 $\pm$ (0.199)&2.61 $\pm$ (0.624)&1.791 $\pm$ (0.652)&1.883 $\pm$ (0.652)\\
\multicolumn{1}{l||}{Contrast Ratio [$DL$]} & 98.744 $\pm$ (0.356)&97.452 $\pm$ (2.028)&98.656 $\pm$ (0.694)&98.576 $\pm$ (0.902)\\
\multicolumn{1}{l||}{Weber Contrast Score [$DL$]} & -1.256 $\pm$ (0.356)&-2.548 $\pm$ (2.028)&-1.344 $\pm$ (0.694)&-1.424 $\pm$ (0.902)\\
\multicolumn{1}{l||}{Michelson Contrast Score [$DL$]} & 95.815 $\pm$ (1.62)&98.09 $\pm$ (2.317)&98.909 $\pm$ (0.686)&98.474 $\pm$ (1.454)\\
\multicolumn{1}{l||}{RMS Contrast Score [$DL$]} & 71.708 $\pm$ (10.515)&70.472 $\pm$ (12.089)&58.318 $\pm$ (17.223)&60.847 $\pm$ (17.007)\\
\multicolumn{1}{l||}{Blurring Percentage  [$\%$]} & 15.357 $\pm$ (9.655)&15.789 $\pm$ (16.718)&47.263 $\pm$ (21.188)&41.048 $\pm$ (23.492)\\
\multicolumn{1}{l||}{Blurring Score [$DL$]} & 798.177 $\pm$ (321.642)&417.948 $\pm$ (290.689)&741.84 $\pm$ (693.735)&724.348 $\pm$ (643.288)\\
\multicolumn{1}{l||}{Local Blurring ($>$0\%) [$\%$]} & 100.0 $\pm$ (0.0)&100.0 $\pm$ (0.0)&100.0 $\pm$ (0.0)&100.0 $\pm$ (0.0)\\
\multicolumn{1}{l||}{Blurred Images ($>$ 50\%) [$\%$]} & 0.677 $\pm$ (2.89)&5.763 $\pm$ (7.598)&61.408 $\pm$ (23.663)&29.471 $\pm$ (33.876)\\
\multicolumn{1}{l||}{Global Blurring ($>$90\%) [$\%$]} & 0.0 $\pm$ (0.0)&0.055 $\pm$ (0.182)&0.995 $\pm$ (1.251)&0.467 $\pm$ (0.975)\\
\multicolumn{1}{l||}{No. SIFT Features [$Features$]} & 2483.223 $\pm$ (1014.512)&1340.838 $\pm$ (922.25)&798.177 $\pm$ (640.056)&1042.4 $\pm$ (907.165)\\
\multicolumn{1}{l||}{Abs. Spatial Dist. - SIFT [$\%$]} & 65.581 $\pm$ (13.022)&41.502 $\pm$ (10.355)&14.546 $\pm$ (10.68)&22.732 $\pm$ (20.551)\\
\multicolumn{1}{l||}{Avg. Spatial Dist. - SIFT [$\%$]} & 60.752 $\pm$ (18.419)&32.798 $\pm$ (13.078)&14.357 $\pm$ (10.207)&21.343 $\pm$ (19.346)\\
\multicolumn{1}{l||}{No. ORB Features [$Features$]} & 9301.195 $\pm$ (2817.107)&4598.831 $\pm$ (3153.477)&3730.404 $\pm$ (2976.571)&4468.376 $\pm$ (3477.047)\\
\multicolumn{1}{l||}{Abs. Spatial Dist. - ORB [$\%$]} & 53.586 $\pm$ (9.634)&38.549 $\pm$ (9.631)&17.964 $\pm$ (11.888)&23.81 $\pm$ (16.813)\\
\multicolumn{1}{l||}{Avg. Spatial Dist.- ORB [$\%$]} & 37.357 $\pm$ (13.075)&28.208 $\pm$ (9.752)&14.988 $\pm$ (8.324)&18.681 $\pm$ (11.975)\\
\multicolumn{1}{l||}{No. FAST Features [$Features$]} & 8601.271 $\pm$ (3042.455)&3652.139 $\pm$ (2532.28)&2702.625 $\pm$ (2490.08)&3486.277 $\pm$ (3200.21)\\
\multicolumn{1}{l||}{Abs. Spatial Dist. - FAST [$\%$]} & 59.484 $\pm$ (11.107)&48.231 $\pm$ (13.635)&28.298 $\pm$ (19.164)&33.56 $\pm$ (21.066)\\
\multicolumn{1}{l||}{Avg. Spatial Dist. - FAST [$\%$]} & 51.194 $\pm$ (11.968)&35.433 $\pm$ (11.703)&22.784 $\pm$ (12.143)&27.164 $\pm$ (15.377)\\
\multicolumn{1}{l||}{Disparity Mean (BM) [$DL$]} & 40.968 $\pm$ (7.73)&87.85 $\pm$ (18.601)&63.289 $\pm$ (9.996)&62.435 $\pm$ (14.772)\\
\multicolumn{1}{l||}{Disparity Std. Dev. (BM) [$DL$]} & 42.271 $\pm$ (9.829)&59.993 $\pm$ (9.948)&51.155 $\pm$ (8.775)&50.745 $\pm$ (9.81)\\
\multicolumn{1}{l||}{Disparity Mean (SGBM) [$DL$]} & 41.02 $\pm$ (9.695)&82.31 $\pm$ (21.405)&58.026 $\pm$ (10.608)&57.793 $\pm$ (14.673)\\
\multicolumn{1}{l||}{Disparity Std. Dev. (SGBM) [$DL$]} & 48.387 $\pm$ (11.073)&59.239 $\pm$ (16.355)&44.888 $\pm$ (11.095)&46.387 $\pm$ (12.188)\\
\multicolumn{1}{l||}{Dist to Closest Match [$Samples$]} & 113.606 $\pm$ (495.024)&3.262 $\pm$ (37.569)&5.948 $\pm$ (97.476)&18.751 $\pm$ (196.428)\\
\multicolumn{1}{l||}{Image Similarity Score [$DL$]} & 0.093 $\pm$ (0.045)&0.186 $\pm$ (0.118)&0.144 $\pm$ (0.044)&0.141 $\pm$ (0.058)\\
\bottomrule
\end{tabular}
}
\caption{Visual Characterization Metrics}
\end{subtable}
\end{table}

==> temp_fig_imu.tex <==
\begin{figure}
\centering

\begin{tikzpicture}

% summation node
\node   [   draw,
            circle,
            minimum size=0.6cm,
        ] (sum) at (0,0){};

\draw   (sum.north east) -- (sum.south west) 
        (sum.north west) -- (sum.south east);

\node[left=-1pt] at (sum.center){\tiny $+$};
\node[below] at (sum.center){\tiny $-$};
\node[above] at (sum.center){\tiny $-$};


% R_b_l node
\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        left=0.5cm of sum
]  (r_mat) {$R_b^l$};

\node[draw, 
        above= 0.5cm of sum,
        align=center
    ] (cr_effect) {Coriolis};


\node [draw,
        minimum width=0.5cm,
        minimum height=1cm,
        right=0.5cm of sum
]  (f_int_1) {$\int$};

\node [draw,
        minimum width=0.5cm,
        minimum height=1cm,
        right=0.5cm of f_int_1
]  (f_int_2) {$\int$};


\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        left=1.5cm of r_mat,
        fill=RedOrange,
]  (acc) {$f^b$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=1.5cm of acc,
        fill=RedOrange,
]  (gyro) {${\omega}^b$};

\node [draw,
        minimum width=0.5cm,
        minimum height=0.5cm,
        below=0.5cm of sum
]  (g_mat) {$g^l$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        right=0.5cm of f_int_2,
        fill=LimeGreen,
]  (position) {$P^l$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=0.2cm of position,
        fill=LimeGreen,
]  (velocity) {$V^l$};



\node   [   draw,
            circle,
            minimum size=0.6cm,
            right=0.5cm of gyro
        ] (sum2) {};

\node [draw,
        minimum width=0.5cm,
        minimum height=1cm,
        below=1.5cm of r_mat
]  (w_int) {$\int$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=1.5cm of f_int_1
]  (r_mat2) {$R_b^l$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=1.5cm of position,
        fill=LimeGreen,
]  (orientation) {${\Theta}^l$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        above=0.5cm of sum2
]  (b_mat) {$R_l^b$};

\node [draw,
        minimum height=1cm,
        minimum width=0.5cm,
        left=0.39cm of b_mat
]  (w_e) {${\omega}_e^l$};


\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=0.3cm of r_mat2
]  (w_diff_1) {$\frac{d}{dt}$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        left=0.5cm of w_diff_1
]  (w_diff_2) {$\frac{d}{dt}$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        above=3.5cm of r_mat2
]  (f_diff_1) {$\frac{d}{dt}$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        left=0.5cm of f_diff_1
]  (f_diff_2) {$\frac{d}{dt}$};


\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=0.3cm of orientation,
        fill=Cyan,
]  (phi) {${\varphi}^b$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        below=0.1cm of phi,
        fill=Cyan,
]  (alpha) {${\alpha}^b$};


\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        above=3.5cm of orientation,
        fill=Cyan,
]  (snap) {${S}^b$};

\node [draw,
        minimum width=1cm,
        minimum height=1cm,
        above=0.1cm of snap,
        fill=Cyan,
]  (jerk) {${J}^b$};

\draw   (sum2.north east) -- (sum2.south west) 
        (sum2.north west) -- (sum2.south east);
\node[left=-1pt] at (sum2.center){\tiny $+$};
\node[above] at (sum2.center){\tiny $-$};

%%% drawing the arrows
\draw[-stealth] (r_mat.east) -- (sum.west) 
    node[midway,above]{$f^l$};

\draw[-stealth] (sum.east) -- (f_int_1.west) 
    node[midway,above]{$f^l_c$};

\draw[-stealth] (f_int_1.east) -- (f_int_2.west) 
    node[midway,above](int_1_out){};

\draw [stealth-] (sum.south) -- (g_mat.north);

\draw[-stealth] (acc.east) -- (r_mat.west);

\draw[-stealth] (cr_effect.south) -- (sum.north);

\draw[-stealth] (f_int_2.east) -- (position.west);
\draw[-stealth] (f_int_1.south) |- (velocity.west);


\draw [-stealth] (gyro.east) -- (sum2.west);

\draw[-stealth] (sum2.east) -- (w_int.west);

\draw[-stealth] (w_int.east) -- (r_mat2.west) 
    node[midway,above]{$\theta^b$};

\draw[-stealth] (w_int.north) -- (r_mat.south);
\draw[-stealth] (r_mat2.east) -- (orientation.west);

\draw[-stealth] (b_mat.south) -- (sum2.north);
\draw[-stealth] (w_e.east) -- (b_mat.west);


\draw[-stealth] (acc.north) |- (f_diff_2.west);
\draw[-stealth] (gyro.south) |- (w_diff_2.west);

\draw[-stealth] (f_diff_2.east) -- (f_diff_1.west);
\draw[-stealth] (w_diff_2.east) -- (w_diff_1.west);

\draw[-stealth] (f_diff_1.east) -- (snap.west);
\draw[-stealth] (w_diff_1.east) -- (phi.west);

\draw[-stealth] (f_diff_2.north) |- (jerk.west);
\draw[-stealth] (w_diff_2.south) |- (alpha.west);

\end{tikzpicture}
\caption{IMU Flow}
\end{figure}

==> visual_char.tex <==
\section{Visual Data Characterization}
Visual sensors is the most commonly used sensors in the SLAM datasets literature. This is a direct indication of their importance and the implicit indication of the utilization of vision as a basic and fundamental building block SLAM. Visual information is rich in nature and provides many insights into the scene a SLAM system is deployed in. Thus, in the proposed framework, a number of characterization metrics were picked based on their direct impact on the front-end sub-system of SLAM \cite{cadena2016past}, and also based on the claimed qualitative characteristics of proposed SLAM dataset. The generic nature of our proposed framework is a key feature of it, and is a key enabler for future extension and alteration of characterization metric with limited development efforts. 

% =====================================================================================================
\subsection{Image Brightness}
Image brightness is one of the metrics that can pose a challenge on SLAM algorithms, specially when it is biased or skewed. A number of operators are being used the academia and the industry to calculate the brightness of each pixel in an image. Some of these operators, their differences, and their limitations were mentioned and discussed in \cite{bezryadin2007brightness} such as arithmetic mean, HSV color scheme, BCH color scheme, and YUV color scheme. \\

In our proposed framework, we depend on the openCV library's definition of brightness which depends on the definition of Luma used in image compression, which is given by:
\begin{equation}
Br = 0.299*R+0.587*G+0.114*B
\end{equation}
To have a single brightness characterization metric for the whole image, we calculate the arithmetic mean of all brightness values (grayscale image intensities) and report this value as the average image brightness.\\

On the sequence level, rapid and abrupt changes in image brightness put more challenges into the path of SLAM algorithms, and thus, the characterization of such phenomena is of great importance. The change of brightness can be characterized by calculating the first-order time derivative of image brightness values $\frac{d Br}{dt}$. A new variable $\beta_Br$ is defined to be the zero-mean first-order time-derivative of brightness and is given by:
\begin{equation}
\beta_{Br} = dBr\dt - \mu_{Br}
\end{equation}
This zero-mean rate of change of image brightness $\beta_Br$ is examined whether it exceeds the values of $|\sigma|$, $|2\sigma|$, and $|3\sigma|$. The number of samples exceeding each threshold are counted and the ratios of the changes w.r.t. the size of the sequence are calculated.

% =====================================================================================================
\subsection{Image Exposure}
Image exposure is an indication of the quality of the lighting condition of the image. To measure image exposure and to detect whether an image is either properly-exposed, over-exposed, or under-exposed, the image intensity histogram is constructed. Then, the mean $\mu$, variance $\sigma$, and skewness $S$ values are calculated. Due to the fact that images may have some pixels with extreme intensity values, we utilize the concept of \textit{trimmed mean} instead of the \textit{arithmetic mean}, which mandates dropping a percentage of pixels $\alpha$ with extreme intensity values present on the two ends of the histogram. The \textit{trimmed mean} is defined by\cite{rice2006mathematical} to be: 
\begin{equation}
\mu_{\alpha} = \frac{1}{n-2[n\alpha]} \sum\limits_{i=n-[n\alpha]}^{[n\alpha+1]} I_i
\end{equation}

Subsequently, the standard deviation and the skewness can be defined as: 
\begin{equation}
\sigma_{\alpha} = \sqrt{\frac{\sum\limits_{i=n-[n\alpha]}^{[n\alpha+1]} (I_i - \mu_{\alpha})}{n-2[n\alpha]} }
\end{equation}

\begin{equation}
S_{\alpha} = \frac{\sum\limits_{i=n-[n\alpha]}^{[n\alpha+1]} (I_i - \mu_{\alpha})^2}{(n-2[n\alpha]-1)*\sigma_{\alpha}^3}
\end{equation}

%As shown in Fig. \ref{fig:detect_exposure}, a bias in the location of the trimmed mean $\mu_{\alpha}$ can be one indication of the improper exposure of the image. Also, the selectivity of the trimmed standard deviation $\sigma_{alpha}$ and the signal skewness adds more emphasis on the detected anomaly. The objective is to detect whether an image is properly exposed, over-exposed, or underexposed. For that purpose, the image intensities histogram is divided into 7 regions: two discarded regions, each representing 5\% of the dynamic range, that are of extreme intensities and five intensity regions, each representing 18\% of the intensities dynamic range. 
In Fig. \ref{fig:exposure_bd}, the exposure level detection mechanism is described. The intensity histogram is divided into seven different zones. For each image, values of the trimmed mean $\mu_{\alpha}$ and the skewness $S_{\alpha}$ are examined. An under-exposed image is defined to have a positive $S_{\alpha}$ and a zone \#1 $\mu_{\alpha}$. An over-exposed image is defined to have a negative $S_{\alpha}$ and a zone \#5 $\mu_{\alpha}$. Locating $\mu_{\alpha}$ in inbetweener zones is an indication of a properly exposed image.

\begin{equation}
Exposure_{Status} = 
\begin{cases}
	BL,					& \mu_{\alpha} \in Zone\#0 \\
    UE, 				& S_{\alpha} > 0 \: \& \: \mu_{\alpha} \in Zone\#1 \\
    OE, 				& S_{\alpha} < 0 \: \& \: \mu_{\alpha} \in Zone\#5 \\
    WL,					& \mu_{\alpha} \in Zone\#6 \\
    PE,              	& \text{otherwise}
\end{cases}
\end{equation}

Where $BL$, $UE$, $OE$, $WL$, and $PE$ refer to black image, under-exposed, over-exposed, white image, and properly-exposed image status.
% =====================================================================================================
\subsection{Image Contrast}
Intuitively, image contrast $C$ is a property of that represents the differences in pixels' colors and brightness. These differences play a vital role in making these images both identifiable and distinguishable. Quantitative measurement of image contrast is a long discussed problem in the literature, however, there exist a number of definitions, outlined and discussed in \cite{peli1990contrast}, that are practically used, which are: The \textit{Contrast Ratio}, \textit{Weber Formula}, \textit{Michelson Formula}, and \textit{root-mean square (RMS)}. The four metrics are given by:

\begin{equation}
C_{CR} = \frac{L_{target}}{L_{background}} *100
\end{equation}

\begin{equation}
C_{W} = \frac{L_{target}- L_{background}}{L_{background}} * 100
\end{equation}

\begin{equation}
C_{M} = \frac{L_{max} - L_{min}}{L_{max} + L_{min}}
\end{equation}

\begin{equation}
C_{RMS} = {[\frac{1}{n} \sum_{i=1}^{n} (l_i - \bar{l})^{2]}}^{\frac{1}{2}}
\end{equation}

Where: $L_{max}$, $L_{min}$, and $L_{background}$ are the maximum, minimum, and background luminance values in the image extracted from the image after the conversion to the LAB colorspace. $l_i$ is the pixel intensity at pixel $i$, and $\bar{l}$ is the normalized mean of the image pixels' intensities.\\

The methods used measure the ration of luminance change in the image w.r.t. the background luminance. However, they differ in the dynamic range in which the output is provided and in the corner cases where they provide unexpected behaviour. The suitability of these methods for measuring contrast is also a long discussed issues in the literatures. For instance, having one pixel with extreme intensity values can bias the contrast measurement, which is not a proper representation of image contrast. However, we believe that the contrast measurements shall be evaluated w.r.t. the application. In the SLAM case, having pixels with extreme values can impact the reliability of some SLAM components such as feature matching and tracking unless some pre-processing is done. Thus, using the contrast measurement to indicate such anomalies has its usefulness in the SLAM context.

% =====================================================================================================
\subsection{Image Blurring}
Motion blurring can result from the motion of either the camera or the objects inside the camera's field of view. In the former case, motion blur is global and its impact shall be manifested on the whole image, while in the later case, local blurring of specific objects in the image can be witnessed. Consequently, the detection of each type of image blurring is different and both are important characterization metrics as they pose two different types of challenges on SLAM when faced with such situations. 
Many blur detection algorithms and techniques are proposed in the literature and are summarized in \cite{pertuz2013analysis}. The techniques mentioned in this work differ in terms of the limitations, the suitability for both local and global blur detection, and in terms of the tunable hyper-parameters impacting the performance. One of the simplest, yet effective, methods; is measuring the variance of the image after applying a high-pass filter on it. This depends on the assumption that blurring detection is synonymous to the lack of edges, which information are present in the high-frequency spectrum of the image. In openCV, applying the Laplacian operator $\nabla^2$ is equivalent to applying a high-pass filter on the image. The Laplacian of an image $I$ can be given by:

\begin{equation}
\nabla^2 = \frac{\partial^2 I}{\partial x^2}.\frac{\partial^2 I}{\partial y^2}
\end{equation}

Subsequently, the variance of the Laplacian operator can be given by:
\begin{equation}
\sigma_{\nabla^2} = \frac{\sum_{i=1}^{N}(\nabla^2_i - \bar{\nabla^2}}{N-1})
\end{equation}
Where $N$ is the number of pixels of the image.

In order to detect whether a given image is considered blurred or not, the variance of Laplcian score must be compared to a programmable threshold $threshold_{blur}$. Similarly, the same concept can be applied to detect local blurring by dividing a given image $I$ into a number of sub-images with a user-defined dimension $d_{si}$. The same operator and thresholding mechanism can be applied on sub-images and thus locate localized blurring.

The resulting matrix of blurring scores of sub-images can further be utilized to detect the percentage of blurring in images. Moreover, the declaration of an image being blurred or not is now subject to the number of blurred sub-images. In the proposed framework, an image is considered blurred if more than $90\%$ of its sub-images are blurred. The details of the process is illustrated in Fig. \ref{fig:Blur_BD}.

This algorithm has some limitation due to its sensitivity to the value of the threshold $threshold_{blur}$ and the nature of the scene we wish to characterize. For instance feature-less scenes such as clear skies cannot be characterized by the aforementioned measure. However, with the combination with other metrics (e.g. detectable visual features metrics), one can identify the reliability of the blurring score and results provided. 
% =====================================================================================================
%\input{tables/ds_analysis_metrics.tex}
% =====================================================================================================
\subsection{Detectable Visual Features}
A fundamental building block in visual SLAM is features extraction and matching. The process starts with features extraction and matching between subsequent images using one of the famous features extractors such as SIFT \cite{lowe2004distinctive}, SURF \cite{bay2006surf}, ORB \cite{rublee2011orb} ...etc. Motion estimation can be performed with a limited number of keypoint matches, however, with more feature matches, the motion estimation process becomes over-constrained, resulting in better estimation accuracy. Subsequently, the measurement of the number of detectable features in datasets and their spatial distribution across the image is needed to indicate the level of challenge a dataset proposes.

On the image level, three visual features extractors are utilized which are: SIFT \cite{lowe2004distinctive}, FAST \cite{rosten2006machine}, and ORB \cite{rublee2011orb} to report the total number of detectable visual features in an image. Then, the image is divided into square-shaped bins with configurable dimensions. Then, the average number of features per bin is calculated, which is given by: 

\begin{equation}
F_{avg} = \frac{F_{total}}{\lceil{I_H/b_{dim}}\rceil * \lceil{I_W/b_{dim}}\rceil}
\label{F_avg_equ}
\end{equation}

Where: $F_{avg}$ is the average features per bin, $F_{total}$ is the total number of detectable features in an image, $I_H$ and $I_W$ are the height and width of the image, and $b_{dim}$ is the configurable dimension of the image bin.

After that, the number of features in each bin $F_{b}$ is compared to the average number of features per bin $F_{avg}$ to detect whether the features are uniformly distributed or spatially biased in the image. If the number of features in a certain bin is greater than or equal to the average number of features per bin, then, the bin is marked to have a proper number of features. The number of bins with features that are greater than or equal to the average number of features per bin $F_{avg}$ are then counted to calculate the percentage of bins with above average detectable features count using the following formula: 

\begin{equation}
F_{dist-avg} = \frac{\sum_{i=1}^{n} \mathbbm{1} (F_i >= F_{avg})}{b_{total}} \% 
\end{equation}

Additionally, the number of bins with any number of features are also counted as anther indication of how well the features are spatially distributed
\begin{equation}
F_{dist-abs} = \frac{\sum_{i=1}^{n} \mathbbm{1} (F_i >= 1)}{b_{total}} \% 
\end{equation}
Where: $F_{dist-avg}$ is the percentage of image with a number of detectable features greater than or equal to the average number of features per pin, $F_{dist-avg}$ is the percentage of detectable features greater than or equal to $1$, $F_i$ is the number of features in a certain bin, $F_{avg}$ is the calculated average number of features per block from equ. \ref{F_avg_equ}, and $b_{total}$ is the total number of bins available in an image. In Fig. \ref{fig:detect_f}, an image from sequence no. 0 in KITTI odometry dataset \cite{geiger2012we} and the SIFT \cite{lowe2004distinctive} features were used to illustrate the process. 
% =====================================================================================================
\subsection{Image Disparity Levels}
Many SLAM solutions support stereo vision due to its usefulness in the detection of image depth and the lack of problem of scale ambiguity \cite{scaramuzza2011visual}. Consequently, most of the datasets provide stereo vision data. One of the challenges a SLAM solution face is the range of disparity values, which is directly related to the depth, given by the following equation:
\begin{equation}
Disparity = x - x' = \frac{Bf}{Z}
\end{equation}

Where $x$, $x'$ are the 2D projections of a 3D point in two stereo image pair, $B$ is the baseline between the two stereo camera, $f$ is the focal length of the camera, and finally $Z$ is the depth of the 3D point. 

In order to characterize the range of disparity values, we calculate the disparity image of the input image pairs and report the average image disparity $\mu_{Disparity}$ and the standard deviation $\sigma_{Disparity}$ of each resulting disparity image. Two different algorithms were used in order to diversity the characterization process which are: the Block Matching algorithm (StereoBM in OpenCV) \cite{konolige2010projected} and the Semi-Global Block Matching algorithm (StereoSGBM in OpenCV)\cite{hirschmuller2007stereo}. Similar parameters were provided to both algorithms in order to ensure the fairness of comparison.
% =====================================================================================================
\subsection{Revisit Frequency and Image Similarity}
A wide range of visual SLAM algorithms depend on the existence of loop-closure opportunities to correct the accumulated errors. In fact, the lack of loop-closure opportunities adds to the challenge a SLAM system has to tackle, and impact the system robustness and resilience when these opportunities are rare or non-existing. Thus, the revisit frequency in SLAM datasets has to be quantitatively measured and reported to expose the dependency of the SLAM solution accuracy on loop-closure. 

A widely-used technique for loop-closure detection is the bag-of-visual-features method, where images are described by a histogram of visual features' frequencies \cite{sivic2003video}. Visual features are called the visual dictionary or the vocabulary and are the result of clustering the visual features space \cite{angeli2008fast}. In the proposed framework, we utilize DBoW2 \cite{GalvezTRO12} which is used by a number of modern state-of-the-art SLAM solutions for loop-closure detection. Moreover, we utilize the visual vocabulary provided with the ORB-SLAM series (ORBVoc) as the base vocabulary for image descriptors due to its diversity.

A number of metrics can be extracted to indicate the level of image similarity in a certain sequence. The DBoW2 \cite{GalvezTRO12} provides a similarity score between queried images. This score, denoted as $LC_S$, is recorded. Additionally, the distance to the closes match, denoted by $LC_D$ and represented in frames, is recorded as indicator of the level of dynamics in the sequence. The calculated score $LC_S$ is checked for three thresholds which are $S=1.0, 0.9, 0.5$ and the number of matches above the aforementioned scores is recorded. In the original DBoW2 \cite{GalvezTRO12} work, a score of $S=0.3$ was considered a successful loop closure opportunity.
